The gradient flow coupling at high-energy and the scale of SU(3) Yang-Mills theory

Using finite size scaling techniques and a renormalization scheme based on the Gradient Flow, we determine non-perturbatively the $\beta$-function of the $SU(3)$ Yang-Mills theory for a range of renormalized couplings $\bar g^2\sim 1-12$. We perform a detailed study of the matching with the asymptotic NNLO perturbative behavior at high-energy, with our non-perturbative data showing a significant deviation from the perturbative prediction down to $\bar{g}^2\sim1$. We conclude that schemes based on the Gradient Flow are not competitive to match with the asymptotic perturbative behavior, even when the NNLO expansion of the $\beta$-function is known. On the other hand, we show that matching non-perturbatively the Gradient Flow to the Schr\"odinger Functional scheme allows us to make safe contact with perturbation theory with full control on truncation errors. This strategy allows us to obtain a precise determination of the $\Lambda$-parameter of the $SU(3)$ Yang-Mills theory in units of a reference hadronic scale ($\sqrt{8t_0}\,\Lambda_{\overline{\rm MS}} = 0.6227(98)$), showing that a precision on the QCD coupling below 0.5\% per-cent can be achieved using these techniques.

==> tables/results_he.tex <==




| wfl | 11 | ele | 5 | 2 |  0.0805(17) | zfl | 11 | ele | 5 | 2 |  0.0798(17) |
| wfl | 11 | ele | 5 | 3 |  0.0815(19) | zfl | 11 | ele | 5 | 3 |  0.0807(18) |
| wfl | 11 | ele | 6 | 2 |  0.0835(26) | zfl | 11 | ele | 6 | 2 |  0.0821(26) |
| wfl | 11 | ele | 6 | 3 |  0.0826(28) | zfl | 11 | ele | 6 | 3 |  0.0813(27) |
| wfl | 11 | mag | 5 | 2 |  0.0819(15) | zfl | 11 | mag | 5 | 2 |  0.0813(15) |
| wfl | 11 | mag | 5 | 3 |  0.0823(16) | zfl | 11 | mag | 5 | 3 |  0.0816(16) |
| wfl | 11 | mag | 6 | 2 |  0.0819(22) | zfl | 11 | mag | 6 | 2 |  0.0809(21) |
| wfl | 11 | mag | 6 | 3 |  0.0810(23) | zfl | 11 | mag | 6 | 3 |  0.0800(23) |
| wfl |  9 | ele | 5 | 2 |  0.0812(14) | zfl |  9 | ele | 5 | 2 |  0.0798(13) |
| wfl |  9 | ele | 5 | 3 |  0.0813(14) | zfl |  9 | ele | 5 | 3 |  0.0798(14) |
| wfl |  9 | ele | 6 | 2 |  0.0824(18) | zfl |  9 | ele | 6 | 2 |  0.0802(18) |
| wfl |  9 | ele | 6 | 3 |  0.0835(22) | zfl |  9 | ele | 6 | 3 |  0.0811(21) |
| wfl |  9 | mag | 5 | 2 |  0.0814(11) | zfl |  9 | mag | 5 | 2 |  0.0803(11) |
| wfl |  9 | mag | 5 | 3 |  0.0814(12) | zfl |  9 | mag | 5 | 3 |  0.0801(12) |
| wfl |  9 | mag | 6 | 2 |  0.0810(15) | zfl |  9 | mag | 6 | 2 |  0.0791(15) |
| wfl |  9 | mag | 6 | 3 |  0.0809(18) | zfl |  9 | mag | 6 | 3 |  0.0789(17) |
| wfl |  7 | ele | 5 | 2 |  0.0830(11) | zfl |  7 | ele | 5 | 2 |  0.0790(10) |
| wfl |  7 | ele | 5 | 3 |  0.0832(12) | zfl |  7 | ele | 5 | 3 |  0.0789(11) |
| wfl |  7 | ele | 6 | 2 |  0.0851(16) | zfl |  7 | ele | 6 | 2 |  0.0787(14) |
| wfl |  7 | ele | 6 | 3 |  0.0858(17) | zfl |  7 | ele | 6 | 3 |  0.0788(16) |
| wfl |  7 | mag | 5 | 2 | 0.08274(92) | zfl |  7 | mag | 5 | 2 | 0.07910(86) |
| wfl |  7 | mag | 5 | 3 | 0.08295(95) | zfl |  7 | mag | 5 | 3 | 0.07902(89) |
| wfl |  7 | mag | 6 | 2 |  0.0834(13) | zfl |  7 | mag | 6 | 2 |  0.0775(12) |
| wfl |  7 | mag | 6 | 3 |  0.0831(14) | zfl |  7 | mag | 6 | 3 |  0.0771(13) |

























